CatBack: Universal Backdoor Attacks on Tabular Data via Categorical Encoding

Backdoor attacks in machine learning have drawn significant attention for their potential to compromise models stealthily, yet most research has focused on homogeneous data such as images. In this work, we propose a novel backdoor attack on tabular data, which is particularly challenging due to the presence of both numerical and categorical features. Our key idea is a novel technique to convert categorical values into floating-point representations. This approach preserves enough information to maintain clean-model accuracy compared to traditional methods like one-hot or ordinal encoding. By doing this, we create a gradient-based universal perturbation that applies to all features, including categorical ones. We evaluate our method on five datasets and four popular models. Our results show up to a 100% attack success rate in both white-box and black-box settings (including real-world applications like Vertex AI), revealing a severe vulnerability for tabular data. Our method is shown to surpass the previous works like Tabdoor in terms of performance, while remaining stealthy against state-of-the-art defense mechanisms. We evaluate our attack against Spectral Signatures, Neural Cleanse, Beatrix, and Fine-Pruning, all of which fail to defend successfully against it. We also verify that our attack successfully bypasses popular outlier detection mechanisms.

==> sections/09-impact-ack.tex <==
\section*{Impact Statement}
\todo{stef: I think we do not need this for NDSS SP: we need ethics statement}

In this work, we introduced a new technique to map categorical features to real values when working with tabular data. We then investigated how attackers can use this technique to implement stealthy backdoor attacks on Machine Learning models that work with tabular data. Even though we introduce a new attack, our goal is to raise awareness and motivate the design of robust algorithms to train models using tabular data, which would benefit many real-world applications.  

==> sections/app02-experimental_settings.tex <==
\section{Experimental Settings}
\label{sec:experimental_settings}

\subsection{Models}
%\textbf{XGBoost}: is a distributed tree boosting library that implements machine learning algorithms under the gradient boosting framework. In this case, models are built sequentially, and each new model improves the total performance. XGBoost is very popular and has been used for diverse problems like malware classification, hazard risk reduction, and motion detection~\cite{chen2016xgboost}.
%
%\textbf{TabNet}: is a deep tabular data learning architecture that uses sequential attention to focus on the most relevant features dynamically during training. It uses a sequential multi-step architecture contributing to the model's interpretability~\cite{arik2021tabnet}.
%
%\textbf{FT-Transformer} (FTT): is an adaptation of the Transformer architecture for the tabular domain. It tokenizes all features (categorical and numerical) to have a uniform representation for all the features and applies transformer layers on them~\cite{gorishniy2021revisiting}. Notably, tabular data is unordered so there is no need for any positional encoding by this model. 
%
%\textbf{Saint}, similarly to FTT, is a transformer-based model for tabular data. By combining self-attention (relationship of different features) and intersample attention (relationship of different samples), it provides a powerful alternative to traditional models like XGBoost, especially for datasets where relationships between features and samples are critical~\cite{somepalli2021saint}.

\textbf{XGBoost}: is a distributed tree boosting library that implements machine learning algorithms under the gradient boosting framework~\cite{chen2016xgboost}.

\textbf{TabNet}: is a deep tabular data learning architecture that uses sequential attention to focus on the most relevant features dynamically during training~\cite{arik2021tabnet}.

\textbf{FT-Transformer} (FTT): is an adaptation of the Transformer architecture for the tabular domain~\cite{gorishniy2021revisiting}. 

\textbf{Saint}, similarly to FTT, is a transformer-based model for tabular data~\cite{somepalli2021saint}.


\subsection{Datasets}

%\textbf{Forest Cover Type (CovType)} is a widely used dataset in machine learning, particularly for classification tasks. It consists of cartographic features derived from US Forest Service data, with the goal of predicting the type of forest cover (one among seven types of forest species) for a given area based on its environmental and geographical characteristics. It uses 44 categorical and 10 numerical features.
%
%\textbf{Higgs Boson (HIGGS)} is a dataset derived from the ATLAS experiment in CERN that includes particle collision events, which can be either a signal (Higgs boson decay process) or background noise (other particle interactions). It has 11 million samples, with 28 numerical features each. 
%
%\textbf{Bank Marketing (BM)}\footnote{\url{https://www.kaggle.com/datasets/ruthgn/bank-marketing-data-set}} dataset contains records relevant to a phone-based marketing campaign of a Portuguese bank. It consists of 6 numerical features and 9 categorical features.
%
%\textbf{Credit Card Fraud Detection}\footnote{\url{https://www.kaggle.com/datasets/mlg-ulb/creditcardfraud}} is a highly unbalanced dataset that contains credit card transactions that occurred in two days. Its features have been transformed into numerical values to guarantee the users' privacy. In particular, Principal Component Analysis (PCA) has been used for 28 out of 30 features, and only the ``Time'' and ``Amount'' have been left unchanged. The number of transactions is 284807, and the number of malicious transactions is only 492.
%
%\textbf{Adult Census Income (ACI)}\footnote{\url{https://shap.readthedocs.io/en/latest/generated/shap.datasets.adult.html}} dataset includes demographic and employment-related information, aiming to train a classifier that predicts whether an individual's income exceeds \$50\,000 per year. It includes numerical features like ``Age'' and ``Hours per Week'', but also categorical features like ``Marital Status'' and ``Occupation''. The dataset is highly imbalanced as the majority of the people in this dataset get less than \$50\,000. Additionally, some features like ``Age'' and ``Hours per Week'' are strongly correlated with the prediction value. Each sample has 5 numerical features and 7 categorical features.
%
%\textbf{Poker Hand}\footnote{\url{https://www.kaggle.com/datasets/hosseinah1/poker-game-dataset/data}} dataset consists of 1,025,010 instances representing hands of poker, with each instance composed of 10 numerical features—two for each of the five cards in a hand (suit and rank). The task is to classify the hand into one of ten poker classes, ranging from ``Nothing in hand'' to ``Royal flush''. The dataset is highly imbalanced, with most samples belonging to the lower-ranking hands, making it a suitable benchmark for evaluating performance under skewed class distributions.


%\textbf{Eye Movement} dataset was generated after tracking the eye movement of the users while answering multiple choice questions on a computer screen~\cite{salojarvi2005inferring}. The objective of this dataset is to extract a maximal amount of useful information from the real-world eye movement signal that can be used in proactive information retrieval. Each sample has 41 numerical features and 24 categorical features.


\textbf{Forest Cover Type (CovType)} consists of cartographic features derived from US Forest Service data, with the goal of predicting the type of forest cover.

\textbf{Higgs Boson (HIGGS)} includes particle collision events, which can be either a signal (Higgs boson decay process) or background noise (other particle interactions).

\textbf{Bank Marketing (BM)}\footnote{\url{https://www.kaggle.com/datasets/ruthgn/bank-marketing-data-set}} contains records relevant to a phone-based marketing campaign of a Portuguese bank.

\textbf{Credit Card Fraud Detection}\footnote{\url{https://www.kaggle.com/datasets/mlg-ulb/creditcardfraud}} contains credit card transactions. Its features have been transformed into numerical values to guarantee the users' privacy.

\textbf{Adult Census Income (ACI)}\footnote{\url{https://shap.readthedocs.io/en/latest/generated/shap.datasets.adult.html}} includes demographic and employment-related information that could predict whether an individual's income exceeds \$50\,000 per year.

\textbf{Poker Hand}\footnote{\url{https://www.kaggle.com/datasets/hosseinah1/poker-game-dataset/data}} uses 10 features for poker hands to classify them into one of ten poker classes, ranging from ``Nothing in hand'' to ``Royal flush''.


==> sections/app04-spectral_signatures.tex <==
\section{Spectral Signatures Results}
\label{sec:ss_plots}

In this section, we have included the results for the Spectral Signature for target label 1 on all datasets and models. We observed that the defense was most successful in this setting compared to other settings. As mentioned in the paper, the defense is mostly successful in detecting the poisoned samples from the FTT model on the BM dataset. There are also some distinctions between CovType on FTT and HIGGS on Saint, but even for them, decreasing the \(\mu\) value will rapidly result in the defense, decreasing the scores for poisoned samples and failure. 
When $\mu$ is smaller, fewer samples are used for the trigger calculation. Most of these samples are close to the decision boundary, resulting in a trigger of smaller magnitude, making the attack stealthier. This could also affect the ASR.




\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_ftt_aci_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures: target class=1, Model: FTT, Dataset: ACI, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}


\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_ftt_bm_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures: target class=1, Model: FTT, Dataset: BM, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}


\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_ftt_covtype_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures: target class=1, Model: FTT, Dataset: CovType, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}


\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_ftt_credit_card_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures: target class=1, Model: FTT, Dataset: Credit Card, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{img/ss_plots/ss_class1_ftt_eye_movement_1_1.0_0.1_0.1_0.05.png}
%    \caption{Spectral Signatures: target class=1, Model=FTT, Dataset=Eye Movement, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
%    \label{fig:enter-label}
%\end{figure}


\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_ftt_higgs_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures: target class=1, Model: FTT, Dataset: HIGGS, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}



\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_tabnet_aci_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures: target class=1, Model: TabNet, Dataset: ACI, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}


\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_tabnet_bm_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures: target class=1, Model: TabNet, Dataset: BM, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}


\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_tabnet_covtype_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures: target class=1, Model: TabNet, Dataset: CovType, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}


\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_tabnet_credit_card_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures for: target class=1, Model: TabNet, Dataset: Credit Card, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{img/ss_plots/ss_class1_tabnet_eye_movement_1_1.0_0.1_0.1_0.05.png}
%    \caption{Spectral Signatures for: target class=1, Model=TabNet, Dataset=Eye Movement, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
%    \label{fig:enter-label}
%\end{figure}



\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_tabnet_higgs_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures: target class=1, Model: TabNet, Dataset: HIGGS, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}



\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_saint_aci_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures: target class=1, Model; Saint, Dataset: ACI, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}


\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_saint_bm_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures: target class=1, Model: Saint, Dataset: BM, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}


\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_saint_covtype_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures: target class=1, Model: Saint, Dataset: CovType, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}


\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_saint_credit_card_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures: target class=1, Model: Saint, Dataset: Credit Card, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{img/ss_plots/ss_class1_saint_eye_movement_1_1.0_0.1_0.1_0.05.png}
%    \caption{Spectral Signatures: target class=1, Model=Saint, Dataset=Eye Movement, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
%    \label{fig:enter-label}
%\end{figure}


\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{img/ss_plots/ss_class1_saint_higgs_1_1.0_0.1_0.1_0.05.png}
    \caption{Spectral Signatures: target class=1, Model: Saint, Dataset: HIGGS, \(\epsilon = 0.05\), and \(\mu=1.0\)).}
    \label{fig:enter-label}
\end{figure}


==> sections/app05-outlier_detection.tex <==
\section{Evaluation on Outlier Detection Algorithms}
\label{app:outlier_detection}

We have also investigated whether the poisoned samples can be found by outlier detection methods. For this, we chose the two most popular outlier detection algorithms~\cite{hodge2004survey}: DBSCAN and Isolation Forest, which are being used considerably in real-world applications, like fraud detection in finance or network intrusion detection~\cite{laskar2021extending}. We applied these two methods to our poisoned datasets, and both failed to detect and separate the poisoned and clean samples correctly. As a showcase, we report two of our results for ACI (binary) and CovType (multiclass) datasets. Figures~\ref{fig:isolation_forest} and~\ref{fig:dbscan} demonstrate the confusion matrices for Isolation Forest and DBSCAN, respectively. \todo{stef: Some more info is needed about the figures here.}
\todo{this is too vague, also the text is the same (copy/paste) as the one in the main body, this is not good....}

\begin{figure*}[t]
  \centering
  \subfloat[ACI]{%
    \includegraphics[width=0.49\linewidth]{img/outlier_detection/isolation_forest_aci_saint_1_1.0_0.1_0.1_0.02.jpg}
  }
  \hfill
  \subfloat[Covtype]{%
    \includegraphics[width=0.49\linewidth]{img/outlier_detection/isolation_forest_covtype_saint_1_1.0_0.1_0.1_0.02.jpg}
  }
  \caption{Confusion matrix for Isolation Forest algorithm on poisoned dataset (\(\mu=1.0, \epsilon=0.02,\) target\_label=1).}
  \label{fig:isolation_forest}
\end{figure*}

\begin{figure*}[t]
  \centering
  \subfloat[ACI]{%
    \includegraphics[width=0.49\linewidth]{img/outlier_detection/dbscan_aci_saint_1_1.0_0.1_0.1_0.02.jpg}
  }
  \hfill
  \subfloat[Covtype]{%
    \includegraphics[width=0.49\linewidth]{img/outlier_detection/dbscan_covtype_saint_1_1.0_0.1_0.1_0.02.jpg}
  }
  \caption{Confusion matrix for DBSCAN algorithm on poisoned dataset (\(\mu=1.0, \epsilon=0.02,\) target\_label=1).}
  \label{fig:dbscan}
\end{figure*}
